Adaptive PBDW approach to state estimation: noisy observations; user-defined update spaces

We provide a number of extensions and further interpretations of the Parameterized-Background Data-Weak (PBDW) formulation, a real-time and in-situ Data Assimilation (DA) framework for physical systems modeled by parametrized Partial Differential Equations (PDEs), proposed in [Y Maday, AT Patera, JD Penn, M Yano, Int J Numer Meth Eng, 102(5), 933-965]. Given $M$ noisy measurements of the state, PBDW seeks an approximation of the form $u^{\star} = z^{\star} + \eta^{\star}$, where the \emph{background} $z^{\star}$ belongs to a $N$-dimensional \emph{background space} informed by a parameterized mathematical model, and the \emph{update} $\eta^{\star}$ belongs to a $M$-dimensional \emph{update space} informed by the experimental observations. The contributions of the present work are threefold: first, we extend the adaptive formulation proposed in [T Taddei, M2AN, 51(5), 1827-1858] to general linear observation functionals, to effectively deal with noisy observations; second, we consider an user-defined choice of the update space, to improve convergence with respect to the number of measurements; third, we propose an \emph{a priori} error analysis for general linear functionals in the presence of noise, to identify the different sources of state estimation error and ultimately motivate the adaptive procedure. We present results for two synthetic model problems in Acoustics, to illustrate the elements of the methodology and to prove its effectiveness. We further present results for a synthetic problem in Fluid Mechanics to demonstrate the applicability of the approach to vector-valued fields.

==> bib_folder/old_bib.tex <==
@book{adams2003sobolev,
  title={Sobolev spaces},
  author={Adams, R A and Fournier, J  JF},
  volume={140},
  year={2003},
  publisher={Academic press}
}

@book{pinkus1985n,
  title={N-widths in Approximation Theory},
  author={Pinkus, A},
  volume={7},
  year={1985},
  publisher={Springer Science \& Business Media}
}


@Book{wiener_filtering,
author = {J. S.  Lim},
publisher = {Prentice Hall},
title = {Two-dimensional signal and image processing},
year = {1990},
}

@article{maday2015pbdw,
  title={PBDW State Estimation: Noisy Observations; Configuration-Adaptive Background Spaces; Physical Interpretations},
  author={Maday, Y and Patera, A  T and Penn, J D and Yano, M},
  journal={ESAIM: Proceedings and Surveys},
  volume={50},
  pages={144--168},
  year={2015},
  publisher={EDP Sciences}
}

@book{hewitt2012abstract,
  title={Abstract Harmonic Analysis: Volume I Structure of Topological Groups Integration Theory Group Representations},
  author={Hewitt, E and Ross, K A},
  volume={115},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@book{hastie2009elements,
  title={The elements of statistical learning},
  author={Hastie, T. and Tibshirani, R. and Friedman, J.},
  volume={2},
  number={1},
  year={2009},
  publisher={Springer}
}

@book{rice2006mathematical,
  title={Mathematical statistics and data analysis},
  author={Rice, J},
  year={2006},
  publisher={Cengage Learning}
}

@book{jacod2003probability,
  title={Probability essentials},
  author={Jacod, J. and Protter, P. E},
  year={2003},
  publisher={Springer}
}
@article{babuska2011optimal,
  title={Optimal local approximation spaces for generalized finite element methods with application to multiscale problems},
  author={Babuska, I  and Lipton, R },
  journal={Multiscale Modeling \& Simulation},
  volume={9},
  number={1},
  pages={373--406},
  year={2011},
  publisher={SIAM}
}

==> sezioni/regularity_result.tex <==
In this note, I address the problem of estimating the $L^{\infty}$ error associated with a Finite Element discretization.
The derivation holds for inf-sup stable elliptic PDEs. Two important references are
the book by Giaquinta and Martinazzi (\cite[Chapter 4]{giaquinta2013introduction}) for some results on interior regularity, and the book by Ciarlet \cite{ciarlet1991basic}.


\subsection{Derivation}

\emph{Notation:}
$u=$ true solution, $u_h=$ FE solution, $a(\cdot, \cdot)=$ inf-sup stable bilinear form,
$\beta=$ inf-sup constant, $\kappa=$ FE order, $V_h=$ FE space.

\begin{theorem}
Let $K$ be an element of the FE mesh such that $K \subset \subset \Omega$.
Let $\widetilde{\Omega}$ be a smooth domain such that
$K \subset  \subset  \widetilde{\Omega}  \subset   \subset   \Omega$.
Then, if $u \in H^2(\widetilde{\Omega})$, the following estimate holds.
\begin{equation}
\label{eq:Linf_est}
\|  u - u_h \|_{L^{\infty}(K)} \leq
\inf_{w_h \in V_h} \,
\left(
 \| u - w_h \|_{L^{\infty}(K)}
+
C(\widetilde{\Omega})  h^{-d/2}   \| u - w_h \|_{L^2(\widetilde{\Omega})}
+
C h^{1-d/2}   \| u - w_h \|_{H^1(\Omega)}
\right),
\end{equation}
where $h$ is the characteristic size of the mesh.
\end{theorem}

\begin{proof}
We need three lemmas.
\begin{enumerate}
\item
$\| u - u_h \|_{H^1(\Omega)} 
\leq \frac{1}{\beta} \inf_{v_h \in V_h} \| v_h - u \|_{H^1(\Omega)} $ (quasi-optimality result);
\item
$\| p \|_{L^{\infty}(K)} \leq C h^{-d/2}  \| p \|_{L^{2}(K)}$
$\forall \, p \in \mathbb{P}^{\kappa}(K)$ where $C=C(\kappa)$.

\emph{Proof (sketch):} In finite dimensions, all norms are equivalent; therefore;
$\| p \|_{L^{\infty}(\hat{K})} \leq C'    \| p \|_{L^{2}(\hat{K})}$ where $\hat{K}$ is the reference element and $C'$ is a function of $\kappa$ and $d$. Thesis follows by applying the change-of-variable formula.
\item
If $u \in H^2(\widetilde{\Omega})$,
then 
$\|  u - u_h \|_{L^2(\widetilde{\Omega})} \leq C h \| u - u_h \|_{H^1(\widetilde{\Omega})}$.

\emph{Proof (sketch):}
The proof is based on the Aubin-Nitsche trick with the only difference that instead of using the adjoint we use
$\phi \in   H_0^1(  \widetilde{\Omega}   )$
$$
a_{\widetilde{\Omega}} (v, \phi) = (u-u_h, v)_{L^2(\widetilde{\Omega})} 
\qquad
\forall \, v \in H_0^1(  \widetilde{\Omega}   ).
$$
\end{enumerate}

The proof of \eqref{eq:Linf_est} relies on a combination of (1-3):
$$
\begin{array}{rl}
\|  u - u_h \|_{L^{\infty}(K)}
\leq
&
\|  u - \tilde{u}_h \|_{L^{\infty}(K)} + \|  u_h - \tilde{u}_h \|_{L^{\infty}(K)} 
\\
\leq &
\|  u - \tilde{u}_h \|_{L^{\infty}(K)} +
C h^{-d/2}   \| u_h - \tilde{u}_h  \|_{L^{2}(K)}  
\\
\leq &
\|  u - \tilde{u}_h \|_{L^{\infty}(K)} + 
C h^{-d/2}  \left( \| u - \tilde{u}_h  \|_{L^{2}(K)} + \|  u - u_h \|_{L^{2}(K)} \right) 
\\
\leq & 
\|  u - \tilde{u}_h \|_{L^{\infty}(K)} 
+ C h^{-d/2}   \| u - \tilde{u}_h  \|_{L^{2}(K)} 
+  C h^{1-d/2}    \|  u - u_h \|_{H^1(K)} 
\\
\leq & 
\|  u - \tilde{u}_h \|_{L^{\infty}(K)} 
+ C h^{-d/2}   \| u - \tilde{u}_h  \|_{L^{2}(K)} 
+  
\frac{1}{\beta}
C h^{1-d/2}    \|  u - \tilde{u}_h \|_{H^1(\Omega)} 
\\
\end{array}
$$
\end{proof}

If $u \notin H^2(\Omega)$,  the result guarantees convergence in 2D, but it does not guarantee convergence in 3D. %My intuition is that the only point of the proof we could actually improve is
% $$
% \| u  - u_h \|_{H^1(\widetilde{\Omega})}
% \leq
% \frac{C}{\beta} \inf_{w_h \in V_h} 
%  \| u  - u_h \|_{H^1( \Omega)}.
% $$
% Improvements would probably lead to the introduction of a suitable weighted Sobolev space.



==> sezioni/temp_algebraic.tex <==
\subsection{Algebraic formulation}
\label{sec:algebraic}

We derive an algebraic formulation for the statement \eqref{eq:PBDW_two_field_formulation};
the derivation is independent of the particular construction of the update space.
Towards this end, given the fields
$z \in \mathcal{Z}_N$ and $\eta \in \mathcal{U}_M$, we introduce the vectors $\mathbf{z} \in \mathbb{R}^N$ and $\boldsymbol{\eta} \in \mathbb{R}^M$ such that
$z = \sum_{n=1}^N z_n \zeta_n$, and $\eta = \sum_{m=1}^M \eta_m \psi_m$,
where $\zeta_1,\ldots,\zeta_N$ and
$\psi_1,\ldots,\psi_M$ are orthonormal bases of $\mathcal{Z}_N$ and $\mathcal{U}_M$, respectively.
Then, we can rewrite \eqref{eq:PBDW_two_field_formulation} as a discrete optimization framework for the coefficients:
\begin{equation}
\label{eq:PBDW_algebraic}
(\mathbf{z}_{\xi}^{\star},  \boldsymbol{\eta}_{\xi}^{\star})
=
{\rm arg} \min_{  (\mathbf{z},  \boldsymbol{\eta}) \in \mathbb{R}^N \times \mathbb{R}^M  }
\,
\xi \|  \boldsymbol{\eta}  \|_2^2
\,
+
\,
\frac{1}{M}
\|   \mathbb{L}_{\eta} \boldsymbol{\eta} + 
 \mathbb{L}_{z} \mathbf{z} - \mathbf{y}  \|_2^2;
\end{equation}
where $\mathbb{L}_z \in \mathbb{R}^{M,N}$, and 
$\mathbb{L}_{\eta} \in \mathbb{R}^{M,M}$ are given by
$(\mathbb{L}_z)_{m,n} = \ell_m^o(\zeta_n)$,
$(\mathbb{L}_{\eta})_{m,m'} = \ell_m^o(\psi_{m'})$.
We observe that   \eqref{eq:unisolvency_update} implies that $\mathbb{L}_{\eta}$ is invertible.
By differentiating the objective function with respect to $\mathbf{z}$ and $\boldsymbol{\eta}$, we obtain
\begin{equation}
\label{eq:PBDW_algebraic_temp}
\left\{
\begin{array}{l}
(\xi M  \mathbb{I} +   \mathbb{L}_{\eta}^T \mathbb{L}_{\eta}     ) \boldsymbol{\eta}_{\xi}^{\star}
+  \mathbb{L}_{\eta}^T \mathbb{L}_{z}  \boldsymbol{z}_{\xi}^{\star}
 =   \mathbb{L}_{\eta}^T    \boldsymbol{y}   \\[4mm]
\mathbb{L}_{z}^T \mathbb{L}_{\eta}  \boldsymbol{\eta}_{\xi}^{\star}
+  \mathbb{L}_{z}^T \mathbb{L}_{z}  \boldsymbol{z}_{\xi}^{\star}
 = \mathbb{L}_{z}^T    \boldsymbol{y}   \\
\end{array}
\right.
\end{equation}
If we multiply \eqref{eq:PBDW_algebraic_temp}$_1$ by $\mathbb{L}_{z}^T  \mathbb{L}_{\eta}^{-T}$, and we exploit \eqref{eq:PBDW_algebraic_temp}$_2$ we obtain
$$
\xi M    \mathbb{L}_{\eta}^T  \mathbb{L}_{\eta}^{-T}  \boldsymbol{\eta}_{\xi}^{\star} + 
\mathbb{L}_{z} ^T \mathbb{L}_{\eta}  \boldsymbol{\eta}_{\xi}^{\star} +
\mathbb{L}_{z}^T \mathbb{L}_{z}  \boldsymbol{z}_{\xi}^{\star}
 =
\mathbb{L}_{z}^T    \boldsymbol{y} 
   =
\mathbb{L}_{z}^T \mathbb{L}_{\eta}  \boldsymbol{\eta}_{\xi}^{\star} +  \mathbb{L}_{z}^T \mathbb{L}_{z}  \boldsymbol{z}_{\xi}^{\star}  
 \Rightarrow
\mathbb{L}_{z}^T \mathbb{L}_{\eta}^{-T}  \boldsymbol{\eta}_{\xi}^{\star}  = \mathbf{0}
$$
Finally, if we introduce $ 
\tilde{ \boldsymbol{\eta}}_{\xi}^{\star} =  
\mathbb{L}_{\eta}^{-T}      \boldsymbol{\eta}_{\xi}^{\star}$ and we multiply \eqref{eq:PBDW_algebraic_temp}$_1$ by $\mathbb{L}_{\eta}^{-T}$, we obtain
\begin{equation}
\label{eq:PBDW_algebraic_linear}
\left\{
\begin{array}{l}
\left( \xi M  \mathbb{I} + \mathbb{L}_{\eta}  \mathbb{L}_{\eta}^{T} \right) \tilde{ \boldsymbol{\eta}}_{\xi}^{\star} 
+ \mathbb{L}_{z}  \boldsymbol{z}_{\xi}^{\star} = \boldsymbol{y}  \\[3mm]
\mathbb{L}_{z}^T  \tilde{ \boldsymbol{\eta}}_{\xi}^{\star}  = \boldsymbol{0}  \\[3mm]
 \boldsymbol{\eta}_{\xi}^{\star} =  \mathbb{L}_{\eta}^{T}   \tilde{ \boldsymbol{\eta}}_{\xi}^{\star}. 
\\
\end{array}
\right.
\end{equation}
System \eqref{eq:PBDW_algebraic_linear} can be used to efficiently compute the PBDW solution.


\begin{remark}
(\textbf{spectrum of the PBDW system})
Following the argument in 
\cite[Section 3.4]{benzi2005numerical}, we observe that
the saddle-point system \eqref{eq:PBDW_algebraic_linear}  is congruent to the block-diagonal matrix 
$\left[
\begin{array}{cc}
\mathbb{L}_{\eta} \mathbb{L}_{\eta}^T  + \xi M \mathbb{I} & 0  \\
0   & - \mathbb{L}_z^T (\mathbb{L}_{\eta} \mathbb{L}_{\eta}^T   + \xi M \mathbb{I})^{-1} \mathbb{L}_z \\
\end{array}
\right]$. 
If the update satisfies \eqref{eq:unisolvency_update}, $\mathbb{L}_{\eta}$ is invertible, and thus 
$\mathbb{L}_{\eta} \mathbb{L}_{\eta}^T  + \xi M \mathbb{I}$ is positive definite for all $\xi \geq 0$.

On the other hand, the second block 
$- \mathbb{L}_z^T (\mathbb{L}_{\eta} \mathbb{L}_{\eta}^T   + \xi M \mathbb{I})^{-1} \mathbb{L}_z$ is negative definite if and only if 
the rank of $\mathbb{L}_z$ is equal to $N$: this condition is equivalent to the positivity of $\beta_{N,M}$ in Proposition \ref{th:variation_empirical_update}.
\end{remark}




\begin{Proposition}
\label{th:well_posedness}
Given the observation functionals $\ell_1^o,\ldots, \ell_M^o \in \mathcal{X}'$,
 the background space $\mathcal{Z}_N={\rm span}\{ \zeta_n \}_{n=1}^N$,
and the update space $\mathcal{U}_M = {\rm span}\{ \psi_m \}_{m=1}^M$ satisfying \eqref{eq:unisolvency_update}, we assume that
\begin{equation}
\label{eq:unisolvency_background}
z \in \mathcal{Z}_N,
\;  \ell_m^o(z) = 0 \; m=1,\ldots,M
\,
\Leftrightarrow
\,
z \equiv 0.
\end{equation}
Then, there exists an unique solution to \eqref{eq:PBDW_two_field_formulation}-\eqref{eq:PBDW_algebraic_linear}.
\end{Proposition}

\begin{proof}
Following the argument in 
\cite[Section 3.4]{benzi2005numerical}, we observe that
the saddle-point system \eqref{eq:PBDW_algebraic_linear}  is congruent to the block-diagonal matrix $\left[
\begin{array}{cc}
\mathbb{L}_{\eta} \mathbb{L}_{\eta}^T  + \xi M \mathbb{I} & 0  \\
0   & - \mathbb{L}_z^T (\mathbb{L}_{\eta} \mathbb{L}_{\eta}^T   + \xi M \mathbb{I})^{-1} \mathbb{L}_z \\
\end{array}
\right]$. 


Since $\mathbb{L}_{\eta}$ is invertible (cf. \eqref{eq:unisolvency_update}),
$\mathbb{L}_{\eta} \mathbb{L}_{\eta}^T  + \xi M \mathbb{I}$ is positive definite for all $\xi \geq 0$.
Similarly, since $\mathbb{L}_{z}$ is full-rank (cf. \eqref{eq:unisolvency_background}),
$- \mathbb{L}_z^T (\mathbb{L}_{\eta} \mathbb{L}_{\eta}^T   + \xi M \mathbb{I})^{-1} \mathbb{L}_z$
is negative definite.
As a result, all the eigenvalues of the saddle-point system  \eqref{eq:PBDW_algebraic_linear}  are non-zero, and the system
is invertible. Thesis follows.
\end{proof}


In view of the analysis of the method, and of the definition of the Greedy procedure for the selection of the observation centers,  next Proposition  provides a computable expression for the inf-sup constant $\beta_{N,M}$ defined in \eqref{eq:inf_sup_constant}.

\begin{Proposition}
\label{th:inf_sup}
Suppose that $\zeta_1,\ldots,\zeta_N$ and $\psi_1,\ldots,\psi_M$ are orthonormal.
The inf-sup constant $\beta_{N,M}$ is the square root of the minimum eigenvalue of the following eigenproblem:
\begin{equation}
\label{eq:inf_sup_algebraic}
\mathbb{L}_z^T \mathbb{W} \mathbb{L}_z \, \mathbf{z}_n
=
\nu_n \left(
\mathbb{I} + 
2 \mathbb{L}_z^T  \mathbb{W} \mathbb{L}_z
- 2  {\rm sym} \left( \mathbb{C}^T \mathbb{L}_{\eta}^{-1} \mathbb{L}_z \right)
\right)
\mathbf{z}_n,
\quad
n=1,\ldots,N;
\end{equation}
where 
$\mathbb{W}  = \mathbb{L}_{\eta}^{-T} \mathbb{L}_{\eta}^{-1}$,
${\rm sym}(A)=\frac{1}{2}(A+A^T)$, and
$\mathbb{C} \in \mathbb{R}^{M,N}$, $\mathbb{C}_{m,n} = (\psi_m, \zeta_n)$.
\end{Proposition}

\begin{proof}
Given $z = \sum_{n=1}^N z_n \zeta_n$, $\eta = \sum_{m=1}^M \eta_m \psi_m$,
we find that 
$\mathcal{I}_M(z) = \sum_{k=1}^M \, \left(   \mathbb{L}_{\eta}^{-1} \mathbb{L}_z \mathbf{z}  \right) \psi_k$. Then, we have
$$
((z, \eta   )) = \mathbf{z}^T \mathbb{L}_z^T \mathbb{W} \mathbb{L}_{\eta} \boldsymbol{\eta},
\quad
\vertiii{\eta}^2 = \boldsymbol{\eta}^T \boldsymbol{\eta};
$$
and
$$
 \vertiii{z}^2 = 
 \|    z  \|^2 +  \|   \mathcal{I}_M(z)  \|^2 - 2 (z, \mathcal{I}_M(z))
+ 
\mathbf{z}^T \mathbb{L}_z^T \mathbb{W} \mathbb{L}_z  \boldsymbol{z}
=
\mathbf{z}^T
\left(
\mathbb{I} + 
2 \mathbb{L}_z^T  \mathbb{W} \mathbb{L}_z
-2  {\rm sym} \left( \mathbb{C}^T \mathbb{L}_{\eta}^{-1} \mathbb{L}_z \right)
\right)
\mathbf{z}.
$$
Therefore, if we introduce
$\mathbb{B} = 
\mathbb{I} + 
2 \mathbb{L}_z^T  \mathbb{W} \mathbb{L}_z
-2  {\rm sym} \left( \mathbb{C}^T \mathbb{L}_{\eta}^{-1} \mathbb{L}_z \right)$, 
and recalling the definition of $\mathbb{W}$,
we find
$$
\beta_{N,M}^2
=
\inf_{\mathbf{z} \in \mathbb{R}^N} \sup_{ \boldsymbol{\eta} \in \mathbb{R}^M  }
\,
\left(
\frac{   
\mathbf{z}^T \mathbb{L}_z^T \mathbb{W} \mathbb{L}_{\eta} \boldsymbol{\eta}
}
{ ( \boldsymbol{\eta}^T  \boldsymbol{\eta} )
\,
\mathbf{z}^T \mathbb{B} \mathbf{z}
}
\right)^2
=
\inf_{\mathbf{z} \in \mathbb{R}^N} 
\,
\frac{   
\mathbf{z}^T \mathbb{L}_z^T \mathbb{W} \mathbb{L}_{z} \mathbf{z}
}
{
\mathbf{z}^T \mathbb{B} \mathbf{z}
}.
$$
Introducing the Lagrangian multiplier $\nu$, we can write the optimality conditions as
$$
\left\{
\begin{array}{l}
\mathbb{L}_z^T \mathbb{W} \mathbb{L}_{z} \mathbf{z} 
=
\nu \mathbb{B} \mathbf{z}  \\[3mm]
\mathbf{z}^T \, \mathbb{B} \mathbf{z}  = 1
\\
\end{array}
\right.
$$
Thesis follows.
\end{proof}

